Analytic Model for Off-Axis GRB Afterglow Images -- Geometry Measurement and Implications for Measuring $H_0$

We present an analytic model for measuring the jet core angle ($\theta_c$) and viewing angle ($\theta_{obs}$) of off-axis gamma-ray bursts independently of the jet angular structure outside of the core. We model the images of off-axis jets and using this model we show that $\theta_{obs}$ and $\theta_c$ can be measured using any two of the three following observables: the afterglow light curve, the flux-centroid motion, and the image width. The model is calibrated using 2D relativistic hydrodynamic simulations with a broad range of jet angular structures. We study the systematic errors due to the uncertainty in the jet structure and find that when using the light curve and centroid motion to determine $\theta_{obs}$ and $\theta_c$, our formulae can be accurate to a level of $5-10\%$ and $30\%$, respectively. In light of the Hubble tension, the systematic error in $\cos\theta_{obs}$ in GRBs originating in a binary compact object merger is of special interest. We find that the systematic uncertainty on the measurement of $\cos\theta_{obs}$ due to the unknown jet structure is smaller than $1.5\%$ for well-observed events. A similar error is expected if the microphysical parameters evolve at a level that is not easily detected by the light curve. Our result implies that this type of systematic uncertainty will not prevent measurement of $H_0$ to a level of $2\%$ with a sample of well-observed GW events with resolved afterglow image motion. Applying our model to the light curve and centroid motion observations of GW170817 we find $\theta_{obs}=19.2\pm 2~\deg$ (1$\sigma$) and $\theta_c=1.5-4~\deg$.

==> other_tex/post_processing.tex <==
In the post-processing code, we calculate for each RHD simulation the images and light curve in the power-law segment $\nu_a,\nu_m<\nu_{obs}<\nu_c$ as seen by observers at different observing angles. We construct observer time arrays, and image grids, and follow by scanning through 
For every frame, we loop through the all mass elements, and for every one consider 400 values of $\phi$, uniformly distributed in $0\le\phi\le \pi$, which correspond to the $x\ge0$.  
The observer frame angles, $\xi$ and $\psi$ are calculated as in \eqref{eq:cosxi} and \eqref{eq:cospsi}.
A mass element in the simulation along with it's $\Delta \phi$ and $\Delta t$ (the lab time between two data dumps) forms a 4-dimensional box, with a non-trivial projection onto the observer time. However, assuming $c\Delta t\gg \Delta r,r\Delta \theta, r\Delta \phi$, we can derive the observer time as the time to which the center of the box is projected, extended only due to the lab-time dimension, $\Delta T = \Delta t\left(1-\beta\cos\xi_v\right)$.

In this method, the box contributes uniformly to $T_-\le T\le T_+$:
\begin{equation}
    T_{\pm} = t - \frac{r}{c}\cos\xi \pm \frac{1}{2}\Delta T
\end{equation}. 
$x$ and $y$ are selected as the cell to which the center of the box contributes, as in equations \eqref{eq:x_obs},\eqref{eq:y_obs}. 

The flux contributed by each sell is calculated following the model in \cite{Sari_piran_Narayan1998}. 

By the definition of $\epsilon_B$, the magnetic field in the shocked fluid is given by:
\begin{equation}
    B=\sqrt{24 \pi \epsilon_B P}
\end{equation}
Where $P$ is the pressure. 
The minimal Lorentz-factor of the power-law electron distribution is:
\begin{equation}
    \gamma_m=\epsilon_e\frac{p-2}{p-1}\frac{3 P m_p}{m_e c^2 \rho}
\end{equation}
and the typical synchrotron frequency is:
\begin{equation}
    \nu_m = \frac{q_e}{2\pi m_e c}\gamma_m^2 B
\end{equation}

The cell luminosity is given by:
\begin{equation}
    \Delta L_{\nu,max} = \frac{m_e c^2 \sigma_T B}{3 q_e m_p}\cdot \gamma \rho r^2\Delta r \sin \theta \Delta \theta \Delta \phi
\end{equation}
where $\gamma\rho$ is the rest frame density, multiplied by the cell volume to give the cell rest-mass. 
To transform to the observer frame we define the Doppler factor:
\begin{equation}
    \delta_D = \frac{1}{\gamma\left(1-\beta\cos\xi_v\right)}
\end{equation}
where $\xi_v$ is the velocity angle to the observer, analogous to $\xi$.
The observer frame flux:
\begin{equation}
    \Delta F_\nu = \Delta L_{\nu,\max}\left(\frac{\nu_{obs}\cdot (1+z)}{\nu_m\delta_D} \right)^\frac{1-p}{2}\cdot \frac{\delta_D^3}{4\pi D_L^2}
    \end{equation}
where $z$ is the red-shift and $d_L$ is the luminosity distance. 
This flux is added to the relevant cell in the image at every observer time between $T_-$ and $T_+$.
